MAUVE: Measuring the Gap Between Neural Text and Human Text using Divergence Frontiers

As major progress is made in open-ended text generation, measuring how close machine-generated text is to human language remains a critical open problem. We introduce MAUVE, a comparison measure for open-ended text generation, which directly compares the learnt distribution from a text generation model to the distribution of human-written text using divergence frontiers. MAUVE scales up to modern text generation models by computing information divergences in a quantized embedding space. Through an extensive empirical study on three open-ended generation tasks, we find that MAUVE identifies known properties of generated text, scales naturally with model size, and correlates with human judgments, with fewer restrictions than existing distributional evaluation metrics.

==> fig/illustration/manifold.tex <==
\begin{tikzpicture}

% draw the surface
% \shade[left color=gray!60,right color=gray!10] 
%   (0,0) to[out=50,in=180] (3.5, 1.25) to[out=75,in=225] (4.5, 3.3) to[out=175,in=25] (1, 2.8) to[out=-135,in=90] (0, 0);
\shade[left color=gray!60,right color=gray!10] 
  (0,0.5) to[out=70,in=105] (3.5, 0.55) to[out=95,in=155] (5.2, 2.3) to[out=115,in=45] (1, 2.7) to[out=-135,in=90] (0, 0.5);
% \shade[left color=gray!60,right color=gray!10] 
%   (0,1) to[out=70,in=105] (2.8, 0.75) to[out=85,in=155] (5.2, 1.7)
%   .. controls (2.8,3.7) and (1.5,3.7) ..  (0, 1); 

% \draw[fill=black] (2.4, 3.2) circle (2pt) ;

% distribution points and line joining them
\draw[thick] (0.8, 2) 
    to[out=60 , in=190] (2.4, 2.9)
    to[out=0,in=150] (3.9, 2.4);

\draw[color=royalazure, fill,rotate around={50:(0.8,2)}] (0.8,2) ellipse (2.1pt and 1pt) node[label={[shift={(0.1,0.15)},text=black]270:{$P$}}] (p_manif) {};
% \draw[color=royalazure!90, fill] (0.8, 2) circle (2pt) node[label={[text=black]270:$P$}] (p_manif) {};
\draw[color=harvardcrimson!90, fill,rotate around={-35:(3.9, 2.4)}] (3.9, 2.4) ellipse (2.2pt and 1.2pt) node[label={[shift={(0.1,0.15)}, text=black]270:$Q$}] (q_manif) {};

\draw[color=oldmauve!90, fill] (2.4, 2.89) ellipse (2.5pt and 1.3pt) node[label={[shift={(0.1,0.15)},text=black]272.5:$R_\lambda$}] (r_manif) {};

% plot P
\node[above = 1.1cm of p_manif](pbox) {
    \begin{tikzpicture}[scale=2]
    % Bounding box
    % \draw (-0.1,-0.1) rectangle (1.24,0.74);
    \draw (0.001, 0.001) rectangle (1,0.7);
    % Function
    \def\normalmixP{\x, {
    0.01 * exp( -((\x-0.19)^2)/ (2 * 0.08 * 0.08) ) + 
    0.65 * exp( -((\x-0.5)^2)/ (2 * 0.08 * 0.08) ) + 
    0.34 * exp( -((\x-0.85)^2)/ (2 * 0.05 * 0.05) )
    }}
    % Plot
    \draw[color=royalazure, preaction={fill=blue!60, fill opacity=0.2}, fill opacity=0.2, pattern=fivepointed stars, pattern color=blue, domain=0.15:1,smooth] (0.15, 0) -- plot (\normalmixP) -- (1, 0);
    % Axes
    % \draw[thick,->] (0,0) -- (1.2,0) node[below, xshift=-1.3cm, yshift=0.1cm] {\tiny Text};
    % \draw[thick,->] (0,0) -- (0,0.7) node[left, rotate=90, xshift=-0.18cm, yshift=0.08cm] {\tiny Probability};
    % \draw[thick,->] (0,0) -- (1.2,0) node[right] {};
    % \draw[thick,->] (0,0) -- (0,0.7) node[above] {};
    % label
    \node at (0.91, 0.47) {$P$};
    \end{tikzpicture}
};

% plot Q
\node[above right= 0.65cm and 0cm of q_manif](qbox) {
\begin{tikzpicture}[scale=2]
    % Bounding box
    \draw (0.001, 0.001) rectangle (1,0.7);
    % Function
    \def\normalmixQ{\x, {
    0.4 * exp( -((\x-0.21)^2)/ (2 * 0.08 * 0.08) ) + 
    0.6 * exp( -((\x-0.59)^2)/ (2 * 0.08 * 0.08) )
    }}
    % plot
    % \draw[color=harvardcrimson,fill=red!15,domain=0:1,smooth] (0, 0) -- plot (\normalmixQ) -- (1, 0);
    \draw[color=harvardcrimson, preaction={fill=red!60, fill opacity=0.2}, fill opacity=0.2, pattern=dots, pattern color=red, domain=0:0.9,smooth] (0, 0) -- plot (\normalmixQ) -- (0.9, 0);
    % axes
    % \draw[thick,->] (0,0) -- (1.2,0) node[below, xshift=-1.3cm, yshift=0.1cm] {\tiny Text};
    % \draw[thick,->] (0,0) -- (0,0.7) node[left, rotate=90, xshift=-0.18cm, yshift=0.08cm] {\tiny Probability};
    % label
    \node at (0.78, 0.46) {$Q$};
    \end{tikzpicture}
};

\draw[->, bend left, dotted, very thick, color=royalazure] (p_manif) to (pbox) ;
\draw[->, bend right, dotted, very thick, color=harvardcrimson] (q_manif) to (qbox.270) ;
\end{tikzpicture}

==> fig/illustration/type-1-2-errors.tex <==
\begin{tikzpicture}[scale=5]
% function defs
\def\normalmixQ{\x, {
0.4 * exp( -((\x-0.21)^2)/ (2 * 0.08 * 0.08) ) + 
0.6 * exp( -((\x-0.59)^2)/ (2 * 0.08 * 0.08) )
}}
\def\normalmixP{\x, {
0.01 * exp( -((\x-0.19)^2)/ (2 * 0.08 * 0.08) ) + 
0.65 * exp( -((\x-0.5)^2)/ (2 * 0.08 * 0.08) ) + 
0.34 * exp( -((\x-0.85)^2)/ (2 * 0.05 * 0.05) )
}}

% Plot
\draw[thick,color=royalazure!70, preaction={fill=blue!60, fill opacity=0.2}, fill opacity=0.2, pattern=fivepointed stars, pattern color=blue, domain=0.15:1.1,smooth] (0, 0) -- (0.15, 0) -- plot (\normalmixP) -- (1, 0);
\draw[thick,color=harvardcrimson!70, preaction={fill=red!60, fill opacity=0.2}, fill opacity=0.2, pattern=dots, pattern color=red, domain=0:0.87,smooth] (0, 0) -- plot (\normalmixQ) -- (0.87, 0) -- (1, 0);

% Axes
\draw[thick,->] (0,0) -- (1.2,0) node[below, xshift=-3.5cm] {\fontfamily{cmss}\selectfont Text};
\draw[thick,->] (0,0) -- (0,0.7) node[left, rotate=90, xshift=-0.8cm, yshift=0.23cm] {\fontfamily{cmss}\selectfont Probability};

% Labels
\node(plabel) at (0.84, 0.38) {$P$};
\node(qlabel) at (0.15, 0.4) {$Q$};

% Text 
\node[draw, align=left, xshift=-2.5cm, yshift=-0.5cm, at=(qlabel), scale=0.8](q_ex_text) {
    \fontfamily{cmss}\selectfont
    \textbf{Type I Error}: \\ 
    The time is \\ the time is \\ the time is \\ the time $\cdots$
};

\node[draw, align=left, xshift=2.3cm, yshift=-0.5cm, at=(plabel), scale=0.8](p_ex_text) {
    \fontfamily{cmss}\selectfont
    \textbf{Type II Error}: \\ 
    I just visited  \\
    Utqiagvik and \\
    Nuchalawoyya \\
    in Alaska.
};

% Example text in plot
\draw[color=harvardcrimson!90, fill] (0.1, 0) circle (0.55pt) {};
\draw[color=royalazure!90, fill] (0.9, 0) circle (0.55pt)  {};

% Arrow from example dot in figure to example text on the side
\draw[->, dotted, very thick, color=harvardcrimson] (0.1, 0) to[out=225, in=300] (q_ex_text.270) {};

\draw[->, dotted, very thick, color=royalazure] (0.9, 0) to[out=300, in=265] (p_ex_text.270) {};


\end{tikzpicture}

